fMPI: Fast Novel View Synthesis in the Wild with Layered Scene Representations

In this study, we propose two novel input processing paradigms for novel view synthesis (NVS) methods based on layered scene representations that significantly improve their runtime without compromising quality. Our approach identifies and mitigates the two most time-consuming aspects of traditional pipelines: building and processing the so-called plane sweep volume (PSV), which is a high-dimensional tensor of planar re-projections of the input camera views. In particular, we propose processing this tensor in parallel groups for improved compute efficiency as well as super-sampling adjacent input planes to generate denser, and hence more accurate scene representation. The proposed enhancements offer significant flexibility, allowing for a balance between performance and speed, thus making substantial steps toward real-time applications. Furthermore, they are very general in the sense that any PSV-based method can make use of them, including methods that employ multiplane images, multisphere images, and layered depth images. In a comprehensive set of experiments, we demonstrate that our proposed paradigms enable the design of an NVS method that achieves state-of-the-art on public benchmarks while being up to $50x$ faster than existing state-of-the-art methods. It also beats the current forerunner in terms of speed by over $3x$, while achieving significantly better rendering quality.

==> pt.tex <==
\subsection{Passthrough application}
Since device-mounted cameras on VR headsets are usually at a significant offset from the users’ eyes, reprojecting video information from such cameras to the eye buffers requires understanding the 3D structure of dynamic scenes and reasoning about (dis-)occlusions from just a small set of input views (see the seminal work of \cite{chaurasia2020passthrough+} for more details on video passthrough (PT)). 



\begin{figure}[h]
    \centering
    \setlength{\tabcolsep}{1.2pt}
    \begin{tabular}{c c}   
        \includegraphics[width=0.499\linewidth, trim=1 1 1 1, clip]{figures/results/npt/npt_results.jpg} &
        \includegraphics[width=0.499\linewidth, trim=1 1 1 1, clip]{figures/results/npt/npt_results.jpg} \\
\multicolumn{1}{c}{NeuralPassthrough} & \multicolumn{1}{c}{fMPI S} \\
    \end{tabular}
    \caption{\textbf{Passthrough:} [DRAFT] Visual comparison between our method and NeuralPassthrough. VIDEO IN SUPPLEMENTARY??}
    \label{fig:npt}
\end{figure}

To show a real world use case for real-time NVS in the wild, we obtain the publically available data captured by the prototype VR headset from \cite{xiao2022neuralpassthrough}. In this set up, two RGB cameras are placed with a baseline of $10cm$. Each camera has a resolution of $1280$x$720$ a $90^{\circ}$ horizontal vertical field of view and square pixels. Recordings are taken for two different indoor scenes (one static and one dynamic). The eye buffers are assumed to have a baseline of $6cm$, positioned $9.3cm$ behind the stereo cameras. Capturing ground truth is hard for closed head-mounted displays and hence there is no training data for this setup. Unfortunately, both spaces and RFF have very different angular resolutions (measured in pixels per FOV degree), which hinders generalization to the captured video streams. For lack of better alternatives, we thus train the synthetic validation dataset released by \citep{xiao2022neuralpassthrough}. This dataset matches the camera setup of the video data, but it consists of only two scenes with $150$ images captured in each.

Figure \ref{fig:npt} shows a visual comparison of our results to the images synthesized by \citep{xiao2022neuralpassthrough}. Clearly, our results are worse which we attribute to the lack of training dataset but we wanted to show a use-case anyway.\footnote{Note that the NeuralPassthrough method employs image-based rendering given stereo depth from a large depth estimation network termed Raft-Stereo \cite{lipson2021raft} which was trained on large synthetic (SceneFlow~\cite{mayer2016large}) and real datasets (Middleburry~\cite{scharstein2014high})}

WHAT ABOUT SPEED: optimize by precomputing homographies and running on lower-res images!!!


